Complete Game Logic with Sabotage

Game Logic with sabotage ($\mathsf{GL_s}$) is introduced as a simple and natural extension of Parikh's game logic with a single additional primitive, which allows players to lay traps for the opponent. $\mathsf{GL_s}$ can be used to model infinite sabotage games, in which players can change the rules during game play. In contrast to game logic, which is strictly less expressive, $\mathsf{GL_s}$ is exactly as expressive as the modal $\mu$-calculus. This reveals a close connection between the entangled nested recursion inherent in modal fixpoint logics and adversarial dynamic rule changes characteristic for sabotage games. A natural Hilbert-style proof calculus for $\mathsf{GL_s}$ is presented and proved complete using syntactic equiexpressiveness reductions. The completeness of a simple extension of Parikh's calculus for game logic follows.

==> preamble.tex <==
\RequirePackage{xspace}
\newcommand{\envelope}[1]{\llbracket#1\rrbracket}

\newcommand{\setcomplement}[2]{{#1}\setminus{#2}}

\newcommand{\grsep}{{}\mid{}}

\newcommand{\patoms}{\mathbb{P}}
\newcommand{\patomsb}{\mathbb{P}_0}
\newcommand{\patomsc}{\mathbb{P}_1}
\newcommand{\patom}{P}
\newcommand{\patomb}{Q}

\newcommand{\gatoms}{\mathbb{G}}
\newcommand{\gatomsd}{\mathbb{G}_1}
\newcommand{\gatomsb}{\mathbb{G}_2}
\newcommand{\gatomsc}{\mathbb{G}_3}
\newcommand{\gatom}{a}
\newcommand{\gatomb}{b}
\newcommand{\gatomc}{c}

\newcommand{\pvars}{\mathbb{V}}
\newcommand{\pvar}{{x}}
\newcommand{\pvarb}{{y}}

\newcommand{\fvar}{\mathsf{u}}
\newcommand{\fvarb}{\mathsf{v}}

\newcommand{\gvars}{\mathbb{V}}
\newcommand{\gvar}{{x}}
\newcommand{\gvarb}{{y}}
\newcommand{\gvarc}{{w}}
\newcommand{\gvarz}{{z}}

\newcommand{\fnot}{\lnot}
\renewcommand{\for}{\lor}
\newcommand{\fand}{\land}
\newcommand{\fandbig}{\bigwedge}
\newcommand{\forbig}{\bigvee}
\newcommand{\fimply}{\limply}
\newcommand{\fequiv}{\lbisubjunct}
\newcommand{\ffalse}{\bot}
\newcommand{\ftrue}{\top}
\newcommand{\flfp}[2]{\mu{#1}.#2}
\newcommand{\fgfp}[2]{\nu{#1}.#2}
\newcommand{\fxfp}[2]{\sigma{#1}.#2}
\newcommand{\flfpstar}[1]{{#1}^*}
\newcommand{\fgfpstar}[1]{{#1}^\times}
\newcommand{\fdia}[2]{\langle{#1}\rangle{#2}}
\renewcommand{\fbox}[2]{[{#1}]#2}
\newcommand{\fid}{\mathrm{id}}
\newcommand{\fcom}{\circ}
\newcommand{\fdual}[1]{{#1}^{\mathrm{d}}}

\newcommand{\gcom}{;}
\newcommand{\gor}{\cup}
\newcommand{\gand}{\cap}
\newcommand{\gtest}[1]{{?{#1}}}
\newcommand{\gdtest}[1]{{\text{\raisebox{2pt}{?`}}{#1}}}
\newcommand{\gdual}[1]{#1^\gduals}
\newcommand{\gdualp}[1]{(#1)^\gduals}
\newcommand{\gstar}[1]{{#1}^*}
\newcommand{\gdstar}[1]{{#1}^\times}
\newcommand{\gstarp}[1]{{(#1)}^*}
\newcommand{\gdstarp}[1]{{(#1)}^\times}

\newcommand{\gduals}{\mathrm{d}}

\newcommand{\gvlfp}[3][]{\glfps_{#1}{(#2)}.(#3)}
\newcommand{\gvgfp}[3][]{\ggfps_{#1}{(#2)}.(#3)}

\newcommand{\glfps}{\mathsf{r}}
\newcommand{\ggfps}{\rotatebox[origin=c]{180}{\ensuremath{\mathsf{r}}}}
\newcommand{\glfp}[2]{\glfps{}#1. #2}{}
\newcommand{\ggfp}[2]{\ggfps{}#1. #2}{}

\newcommand{\glfpunroll}[2]{\freplace{#2}{#1}{\glfp{#1}{#2}}}
\newcommand{\gxfp}[2]{\sigma{#1}.{#2}}
\newcommand{\gxfpunroll}[2]{\freplace{#2}{#1}{\gxfp{#1}{#2}}}

\newcommand{\ffalsee}{\fnot(\fid\for\fnot\fid)}
\newcommand{\ftruee}{\fid\for\fnot\fid}
\newcommand{\fande}[2]{\fnot(\fnot#1\for\fnot#2)}
\newcommand{\fduale}[1]{\fnot#1\fcom\fnot\fid}
\newcommand{\fgfpe}[3][]{\nu^{#1}{#2}.#3}

\newcommand{\fsnot}[1]{\overline{#1}}
\newcommand{\gsnot}[1]{{#1}^{\mathsf{d}}}
\newcommand{\gsnotp}[1]{{(#1)}^{\mathsf{d}}}
\newcommand{\freplace}[3]{#1\tfrac{#3}{#2}}
% \newcommand{\freplacel}[3]{#1[#2\mapsto#3]}
\newcommand{\greplace}[3]{#1\tfrac{#3}{#2}}
\newcommand{\flfpunroll}[3][]{\freplace{#3}{#2}{\flfp[#1]{#2}{#3}}}

\newcommand{\gangelswin}[1]{{\sim}{#1}}
\newcommand{\gdemonswin}[1]{{\sim}{#1^\mathrm{d}}}

\newcommand{\FLCname}{Fixpoint Logic with Chop\xspace}
\newcommand{\Flcname}{Fixpoint logic with chop\xspace}
\newcommand{\flcname}{fixpoint logic with chop\xspace}
\newcommand{\flcnameshort}{\texorpdfstring{\ensuremath{\mathsf{FLC}}}{FLC}\xspace}
\newcommand{\eflcname}{extended fixpoint logic with chop\xspace}

\newcommand{\LMuname}{Modal \mutex-Calculus\xspace}
\newcommand{\lmuname}{modal \mutex-calculus\xspace}
\newcommand{\lmushortname}{\texorpdfstring{\ensuremath{\mathsf{L}_\mu}}{Lmu}\xspace}

\newcommand{\LMustarname}{Modal \asttex-Calculus\xspace}
\newcommand{\lmustarname}{modal \asttex-calculus\xspace}
\newcommand{\lmustarshortname}{\texorpdfstring{\ensuremath{\mathsf{L}_\ast}}{L*}\xspace}

\newcommand{\LMusepname}{Separable Modal \mutex-Calculus\xspace}
\newcommand{\lmusepname}{separable modal \mutex-calculus\xspace}
\newcommand{\lmusepshortname}{\(\mathsf{L}_{s}\)\xspace}

\newcommand{\glname}{game logic\xspace}
\newcommand{\Glname}{Game logic\xspace}
\newcommand{\GLname}{Game Logic\xspace}
\newcommand{\glshortname}{\texorpdfstring{\ensuremath{\mathsf{GL}}}{GL}\xspace}

\newcommand{\glmuname}{recursive game logic\xspace}
\newcommand{\Glmuname}{Recursive game logic\xspace}
\newcommand{\GLmuname}{Recursive Game Logic\xspace}
\newcommand{\glmushortname}{\texorpdfstring{\ensuremath{\mathsf{RGL}}}{RGL}\xspace}

\newcommand{\glrulesgame}{sabotage\xspace}
% \newcommand{\glsname}{sabotage game logic\xspace}
% \newcommand{\Glsname}{Sabotage game logic\xspace}
% \newcommand{\GLSname}{Sabotage Game Logic\xspace}
\newcommand{\glsname}{game logic with sabotage\xspace}
\newcommand{\Glsname}{Game logic with sabotage\xspace}
\newcommand{\GLSname}{Game Logic with Sabotage\xspace}
\newcommand{\glsshortname}{\texorpdfstring{\ensuremath{\mathsf{GL_s}}}{GL}\xspace}

\newcommand{\Glmurlname}{Right-linear game logic\xspace}
\newcommand{\glmurlname}{right-linear game logic\xspace}
\newcommand{\GLmurlname}{Right-linear Game Logic\xspace}
\newcommand{\glmurlshortname}{\texorpdfstring{\ensuremath{\mathsf{rlGL}}}{rlGL}\xspace}

\newcommand{\flcsyntaxnoneg}{
    \fml ::= \fid \grsep \patom \grsep \fnot\patom \grsep \pvar  \grsep \fml \for \fmlb \grsep \fml \fand \fmlb \grsep \fdia{a}{\fml} \grsep \fbox{a}{\fml} \grsep \fml \fcom \fmlb \grsep \flfp{\pvar}{\fml}
    \grsep \fgfp{\pvar}{\fml}
}

\newcommand{\flcsyntax}{
    \fml ::= \fid \grsep \patom \grsep \pvar \grsep \fdia{a}{\fml} \grsep \fnot \fml \grsep \fml \for \fmlb \grsep \fml \fcom \fmlb \grsep \flfp{\pvar}{\fml}
}

\newcommand{\lmusyntaxnonneg}{
    \fml ::= \patom \grsep \fnot\patom \grsep \pvar  \grsep \fml \for \fmlb \grsep \fml \fand \fmlb \grsep \fdia{\gatom}{\fml} \grsep \fbox{\gatom}{\fml} \grsep \flfp{\pvar}{\fml}
    \grsep \fgfp{\pvar}{\fml}
}

\newcommand{\lmustarsyntax}{
    \fml ::= \fid \grsep \patom \grsep \fnot \fml \grsep \fml\for\fmlb \grsep \fdia{\gatom}{\fml} \grsep\fml\fcom\fmlb \grsep \flfpstar{\fml}
}

\newcommand{\lmustarsyntaxnonneg}{
    \fml ::= \fid \grsep \patom \grsep \fnot\patom \grsep \pvar \grsep \fdia{\gatom}{\fml} \grsep \fbox{\gatom}{\fml} \grsep\fml\fcom\fmlb \grsep \flfpstar{\fml} \grsep{\fgfpstar{\fml} }
}

\newcommand{\lmusyntax}{
    \fml ::= \patom \grsep \pvar \grsep \fnot \fml \grsep \fml \for \fmlb \grsep \fdia{\gatom}{\fml} \grsep \flfp{\pvar}{\fml}
}
\newcommand{\lmusyntaxhighlight}{
    \fml ::= \patom \grsep {\color{red}\pvar} \grsep \fnot \fml \grsep \fml \for \fmlb \grsep \fdia{\gatom}{\fml} \grsep {\color{red}\flfp{\pvar}{\fml(\pvar)}}
}

\newcommand{\glsyntax}{
    \fml &::= \patom \grsep \fnot \fml \grsep \fml \for \fmlb \grsep \fdia{\gam}{\fml}
    \\
    \gam &::= \gatom \grsep \gdual{\gam} \grsep \gtest{\fml} \grsep \gam\gor\gamb \grsep \gam\gcom\gamb \grsep \gstar{\gam}
}

\newcommand{\glsyntaxnonneg}{
    \fml &::= \patom \grsep \fnot \fml \grsep \fml \for \fmlb \grsep \fdia{\gam}{\fml}
    \\
    \gam &::= \gatom \grsep \gdual{\gatom} \grsep \gtest{\fml} \grsep \gdtest{\fml} \grsep \gam\gor\gamb \grsep\gam\gand\gamb \grsep \gam\gcom\gamb \grsep \gstar{\gam}\grsep \gdstar{\gam}
}

\newcommand{\glmusyntax}{
    \fml &::= \patom \grsep \fnot \fml \grsep \fml \for \fmlb \grsep \fdia{\gam}{\fml}
    \\
    \gam &::= \gatom \grsep \gvar \grsep \gdual{\gam} \grsep \gtest{\fml} \grsep \gam\gor\gamb \grsep \gam\gcom\gamb \grsep \glfp{\gvar}{\gam}
}

\newcommand{\glmusyntaxnoneg}{
    \fml &::= \patom \grsep \fnot \patom \grsep \fml \for \fmlb \grsep \fml \fand \fmlb \grsep \fdia{\gam}{\fml}
    \\
    \gam &::= \gatom \grsep \gdual{\gatom} \grsep \gvar \grsep \gdual{\gvar} \grsep \gtest{\fml} \grsep \gdtest{\fml} \grsep \gam\gor\gamb \grsep\gam\gand\gamb \grsep \gam\gcom\gamb \grsep \glfp{\gvar}{\gam} \grsep \ggfp{\gvar}{\gam}
}

\newcommand{\glrulessyntaxnonneg}{
    \fml &::= \patom \grsep \fnot \fml \grsep \fml \for \fmlb \grsep \fdia{\gam}{\fml}
    \\
    \gam &::= \gatom \grsep \gdual{\gatom} \grsep \gangelswin{\gatom} \grsep \gdemonswin{\gatom} \grsep \gtest{\fml} \grsep \gdtest{\fml} \grsep \gam\gor\gamb \grsep\gam\gand\gamb \grsep \gam\gcom\gamb \grsep \gstar{\gam}\grsep \gdstar{\gam}
}

\newcommand{\glrulessyntax}{
    \fml &::= \patom \grsep \fnot \fml \grsep \fml \for \fmlb \grsep \fdia{\gam}{\fml}
    \\
    \gam &::= \gatom \grsep \gangelswin{\gatom} \grsep \gdual{\gam} \grsep \gtest{\fml} \grsep \gam\gor\gamb \grsep \gam\gcom\gamb \grsep \gstar{\gam}
}

\newcommand{\glrulessyntaxhighlight}{
    \fml &::= \patom \grsep \fnot \fml \grsep \fml \for \fmlb \grsep \fdia{\gam}{\fml}
    \\
    \gam &::= \gatom \grsep {\color{red}\gangelswin{\gatom}}  \grsep \gtest{\fml} \grsep \gam\gor\gamb \grsep \gam\gcom\gamb \grsep \gstar{\gam}\grsep \gdual{\gam}
}

\newcommand{\wellnamed}{well-named\xspace}

\newcommand{\fml}{\varphi}
\newcommand{\fmlb}{\psi}
\newcommand{\fmlc}{\rho}
\newcommand{\fmld}{\delta}
\newcommand{\fmle}{\gamma}
\newcommand{\fmlaux}{\xi}
\newcommand{\fmlauxb}{\zeta}
\newcommand{\fmlauxc}{\chi}
\newcommand{\Fml}{\Phi}

\newcommand{\gam}{\alpha}
\newcommand{\gamb}{\beta}
\newcommand{\gamc}{\gamma}
\newcommand{\gamd}{\delta}
\newcommand{\gamf}{\eta}

\newcommand{\Ord}{\mathrm{Ord}}
\newcommand{\Ordext}{\overline{\mathrm{Ord}}}
\newcommand{\ord}{\gamma}
\newcommand{\ordb}{\delta}
\newcommand{\ordlim}{\lambda}
\newcommand{\ordlimb}{\kappa}
\newcommand{\pow}[1]{\mathcal{P}(#1)}
\newcommand{\emptyseq}{\varepsilon}

\newcommand{\id}{\mathrm{id}}
\newcommand{\union}{\cup}
\newcommand{\intersection}{\cap}
\newcommand{\Union}{\bigcup}
\newcommand{\Intersection}{\bigcap}

\newcommand{\iffc}{\text{iff}\quad}

\newcommand{\mutex}{\texorpdfstring{$\mu$}{mu}}
\newcommand{\asttex}{\texorpdfstring{$\ast$}{star}}

\newcommand{\nstname}{monotone neighbourhood structure\xspace}
\newcommand{\kstname}{Kripke structure\xspace}

\newcommand{\nst}{\mathcal{N}}
\newcommand{\nstb}{\mathcal{M}}

\newcommand{\kst}{\mathcal{K}}

\newcommand{\nstdom}[1]{|#1|}
\newcommand{\nstnf}[2]{{{#1}({#2})}}
\newcommand{\nstpv}[2]{{{#1}({#2})}}

\newcommand{\nste}[1][\nst]{(\nstdom{#1},\nstpv{#1},\nstnf{#1}{\cdot})}

\newcommand{\semflcf}[3][\nst]{#1\envelope{#3}^{#2}}
\newcommand{\semflcfzero}[3][\nst]{#1\envelope{#3}^{#2}(\emptyset)}
% \newcommand{\semflcfzero}[3][\nst]{#1\envelope{#3}^{#2}_0}
\newcommand{\semglf}[3][\nst]{#1\envelope{#3}^{#2}}
\newcommand{\semglg}[3][\nst]{#1\envelope{#3}^{#2}}
\newcommand{\semglgc}[2][\nst]{#1{}\envelope{#2}_{\mathsf{s}}}
\newcommand{\semglfc}[2][\nst]{#1{}\envelope{#2}_{\mathsf{s}}}
\newcommand{\semglgcva}[3][\nst]{#1{}\envelope{#3}^{#2}_{\mathsf{s}}}
\newcommand{\semglfcva}[3][\nst]{#1{}\envelope{#3}^{#2}_{\mathsf{s}}}
\newcommand{\semglgzero}[2][\nst]{#1\envelope{#2}}
\newcommand{\val}{I}
\newcommand{\valb}{J}
\newcommand{\valcomp}[1]{{#1}^\mathrm{c}}
\newcommand{\valsubst}[3][\val]{#1[{#2}\mapsto{#3}]}
\newcommand{\valname}{valuation\xspace}
\newcommand{\valconst}[2][\val]{#1[#2]}

\newcommand{\cont}{c}
\newcommand{\contb}{e}
\newcommand{\contc}{d}
\newcommand{\contzero}{c_\emptyset}
\newcommand{\contdual}[1]{\overline{#1}}
\newcommand{\contexts}{\mathcal{C}}
\newcommand{\contextname}{context\xspace}
\newcommand{\contmod}[3][\cont]{#1\tfrac{#3}{#2}}
\newcommand{\conlift}[1]{\widehat{#1}}
\newcommand{\nstnflift}[2]{{\widehat{#1}({#2})}}

\newcommand{\contnat}[1]{\contb_{#1}}

\newcommand{\conextcomp}[1]{{#1}^{\mathsf{C}}}
\newcommand{\conextdual}[1]{{#1}^{\mathsf{D}}}

\newcommand{\playernocon}{\mathsf{\emptyset}}
\newcommand{\playeronecon}{\mathsf{\diamond}}
\newcommand{\playertwocon}{{\kern-1pt\raisebox{-1pt}{\rotatebox{45}{${\mathsf{\diamond}}$}}}}

\newcommand{\semequiv}{\equiv}
\newcommand{\synequiv}{\equiv}

\newcommand{\validflcin}[2]{{}#1\vDash #2}
\newcommand{\validflcany}[1]{{}\vDash #1}
\newcommand{\validflcnbhd}[1]{{}\vDash #1}
\newcommand{\validflckripke}[1]{{}\vDash_{K} #1}

\newcommand{\notvalidglmuin}[2]{{}#1\not\vDash #2}
\newcommand{\validglmuin}[2]{{}#1\vDash #2}
\newcommand{\validglmuany}[1][]{{}\vDash #1}
\newcommand{\validglmunbhd}[1][]{{}\vDash #1}
\newcommand{\validglmukripke}[1][]{{}\vDash_{K} #1}

\newcommand{\notvalidglrulesin}[2]{{}#1\not\vDash #2}
\newcommand{\validglrulesin}[2]{{}#1\vDash #2}
\newcommand{\validglrulesany}[1][]{{}\vDash #1}
\newcommand{\validglrulesnbhd}[1][]{{}\vDash #1}
\newcommand{\validglruleskripke}[1][]{{}\vDash_{K} #1}

\newcommand{\xset}{X}
\newcommand{\yset}{Y}
\newcommand{\xel}{r}
\newcommand{\yel}{s}
\newcommand{\xpel}{A}
\newcommand{\ypel}{B}
\newcommand{\zpel}{C}

\newcommand{\nfunc}{p}
\newcommand{\nfuncb}{q}
\newcommand{\nfuncs}[1]{\mathcal{G}(#1)}
\newcommand{\nfuncse}[1]{#1\to\pow{\pow{#1}}}
\newcommand{\nfunctest}[1]{#1_?}
\newcommand{\wregtest}[1]{#1_?}
\newcommand{\wregdual}[1]{#1^\mathrm{d}}
\newcommand{\nfuncdual}[1]{{#1}^\mathrm{d}}

\newcommand{\nfuncconst}[1]{c_{#1}}

\newcommand{\nftonffunc}{F}
% \newcommand{\mfpval}{F}

\newcommand{\wreg}{w}
\newcommand{\wregb}{u}
\newcommand{\wregs}[1]{\mathcal{W}(#1)}
\newcommand{\wregse}[1]{\pow{#1}\to\pow{#1}}

\newcommand{\WRegfuncname}{Effectivity Function\xspace}
\newcommand{\wregfuncname}{effectivity function\xspace}

\newcommand{\atgamename}{atomic game\xspace}
\newcommand{\sabactionname}{sabotage action\xspace}

\newcommand{\wregfnfunc}[1]{\hat{#1}}
\newcommand{\nfuncfwreg}[1]{\check{#1}}

\newcommand{\rightlinear}{right-linear\xspace}
\newcommand{\Rightlinear}{Right-linear\xspace}

\newcommand{\separable}{separable\xspace}

\newcommand{\doublesharp}{{\sharp\llap{\raisebox{-1.5pt}{\rotatebox{18}{ -}}}}}
\newcommand{\doublenatural}{{\natural\llap{\raisebox{-1.5pt}{\rotatebox{18}{ -}}}}}
\newcommand{\doublenaturalb}{{\natural\llap{\raisebox{-1.0pt}{\rotatebox{6}{ -}}}}}

\newcommand{\flctoglmus}{\doublesharp}
\newcommand{\flctoglmu}[1]{{#1}^\flctoglmus}
\newcommand{\flctoglmup}[1]{{(#1)}^\flctoglmus}

\newcommand{\flctoglmufs}{\sharp}
\newcommand{\flctoglmuf}[1]{{#1}^\flctoglmufs}
\newcommand{\flctoglmufp}[1]{{(#1)}^\flctoglmufs}

\newcommand{\flctoflc}[1]{{#1}^{\flctoglmufs\rlglmutoflcs}}
\newcommand{\glmutoglmuf}[1]{{#1}^{\rlglmutoflcs\flctoglmufs}}
\newcommand{\glmutoglmug}[1]{{#1}^{\rlglmutoflcs\flctoglmus}}

\newcommand{\qflat}{\reflectbox{$\flat$}}
\newcommand{\rlglmutoflcs}{\qflat}
\newcommand{\rlglmutoflc}[1]{{#1}^{\rlglmutoflcs}}
\newcommand{\rlglmutoflcp}[1]{{(#1)}^{\rlglmutoflcs}}

\newcommand{\glmutoflcs}{\flat}
\newcommand{\glmutoflc}[1]{{#1}^\glmutoflcs}
\newcommand{\glmutoflcp}[1]{{(#1)}^\glmutoflcs}

\newcommand{\lmseptolmstars}{\ensuremath{F}}
\newcommand{\lmseptolmstar}[1]{{#1}^{\lmseptolmstars}}
\newcommand{\lmseptolmstarp}[1]{{#1}^\lmseptolmstars}

\newcommand{\equiexpressive}{equi-expressive\xspace}

\newcommand{\pvartogvar}[1]{#1}
\newcommand{\gvartopvar}[1]{#1}

\newcommand{\compaxset}[1][\axgatset]{\mathcal{S}_{#1}}
\newcommand{\compaxsettilde}[1][\axgatset]{{\mathrm{S}}_{#1}}

\newcommand{\gset}[1]{{#1}^+}
\newcommand{\gunset}[1]{{#1}^-}
\newcommand{\gconst}[1]{\hat{#1}}
\newcommand{\gmod}[1]{b_#1}
\newcommand{\gmodb}[1]{c_#1}
\newcommand{\gmodns}[1]{b}
\newcommand{\gmodbns}[1]{c}

\newcommand{\rlglmutoglruless}{\doublenatural}
\newcommand{\rlglmutoglrulesus}{\doublenaturalb}
\newcommand{\rlglmutoglrulesfs}{\natural}
\newcommand{\rlglmutoglrules}[1]{{#1}^\rlglmutoglrulesus}
\newcommand{\rlglmutoglrulesp}[1]{{(#1)}^\rlglmutoglrulesus}
\newcommand{\rlglmutoglrulesf}[1]{{#1}^\rlglmutoglrulesfs}
\newcommand{\rlglmutoglrulesfp}[1]{{(#1)}^\rlglmutoglrulesfs}

\newcommand{\glrulestorl}[2]{{{#1}^{#2}}}
\newcommand{\glrulestorlp}[2]{{(#1)}^{#2}}
\newcommand{\glrulesadd}[2]{{#1}^{\hat{#2}}}
\newcommand{\glrulesaddp}[2]{{(#1)}^{\hat{#2}}}
\newcommand{\glrulesexp}[1]{\tilde{#1}}
\newcommand{\glruleschecked}[1]{\widehat{#1}}

\newcommand{\contvar}[1]{\gvarb_{#1}}
\newcommand{\valofcont}[1]{\val_{#1}}

\newcommand{\synsab}[1]{\widehat{#1}}
\newcommand{\synsabp}[1]{\widehat{#1}}

\newcommand{\doublehat}[1]{\widehat{\widehat{#1}}}
\newcommand{\triplehat}[1]{\widehat{\widehat{\widehat{#1}}}}

\newcommand{\synsabb}[1]{#1'}
\newcommand{\synsabbp}[1]{(#1)'}

\newcommand{\synsabbb}[1]{{#1}''}
\newcommand{\synsabbbp}[1]{(#1)''}

\newcommand{\synsabbbb}[1]{{#1}'''}
\newcommand{\synsabbbbp}[1]{(#1)'''}

% \newcommand{\synsabb}[1]{\doublehat{#1}}
% \newcommand{\synsabbp}[1]{\doublehat{{#1}}}
% \newcommand{\synsabb}[1]{{{#1}}^E}
% \newcommand{\synsabbp}[1]{{(#1)}^E} 
% \newcommand{\synsabbb}[1]{\triplehat{{#1}}}
% \newcommand{\synsabbbp}[1]{\triplehat{{#1}}}
% \newcommand{\synsabbbb}[1]{{{#1}^G}}
% \newcommand{\synsabbbbp}[1]{{(#1)}^G}
\newcommand{\guardedsgl}[1]{\check{#1}}

\newcommand{\provlmugs}{\lmushortname}
\newcommand{\provlmums}{\vdash}
\newcommand{\monlmu}{{\mathsf{m}\lmushortname}}

\newcommand{\provlmuany}[2][]{{}#1\vdash#2}
\newcommand{\provlmug}[2][]{{\provlmugs}#1\vdash #2}
\newcommand{\provlmum}[2][]{{\mathsf{m}\lmushortname}#1\vdash#2}

\newcommand{\provrlgls}{\glmurlshortname}
\newcommand{\provrlglany}[2][]{{}#1\vdash_{?}#2}
\newcommand{\provrlglg}[2][]{{\glmurlshortname+G}#1\vdash#2}
\newcommand{\provrlglm}[2][]{{\glmurlshortname}#1\vdash#2}
\newcommand{\provrlglgs}{{\glmurlshortname+G}}

\newcommand{\provglmus}{\glmushortname}
\newcommand{\provglmug}[2][]{{\provglmus+G}#1\vdash#2}
\newcommand{\provglmum}[2][]{{\provglmus}#1\vdash#2}
\newcommand{\provglgmus}{{\provglmus+G}}

\newcommand{\provglm}[2][]{{\glshortname}#1\vdash#2}
\newcommand{\provglgs}{{\glshortname+G}}
\newcommand{\provglg}[2][]{{\provglgs}#1\vdash#2}
\newcommand{\axgatset}{\Gamma}
\newcommand{\provglax}[2][\axgatset]{{}\glshortname+\compaxset[#1]\vdash#2}
\newcommand{\provglaxg}[2][\axgatset]{{}\glshortname+G+\compaxset[#1]\vdash#2}
% \newcommand{\provglaxtilde}[1]{{}\glsshortname+\tilde{\compaxset[#1]}\vdash#1}
\newcommand{\provgls}[1]{{\glsshortname}\vdash#1}
\newcommand{\provglsg}[1]{{\glsshortname+G}\vdash#1}
\newcommand{\provglss}{{\glsshortname}}

\newcommand{\rankname}{rank\xspace}
\newcommand{\Rankname}{Rank\xspace}
\newcommand{\rank}{\mathrm{rank}}

\newcommand{\FV}[1]{\mathsf{FV}{(#1)}}

\newcommand{\sabdual}{sabotage dual\xspace}

\newcommand{\contproj}[2]{#1{\upharpoonright}#2}

\newcommand{\simalt}[1]{\tilde{#1}}
\newcommand{\contsetgam}[1]{\eta_{#1}}
% \newcommand{\contsetgamb}[1]{\zeta_{#1}}
% \newcommand{\contcheckgam}[1]{\xi_{#1}}
\newcommand{\contcheckgam}[1]{\sabread[\scvar]{#1}}
\newcommand{\contsetgamb}[1]{\sabset[\scvar]{#1}}

\newcommand{\contvarfp}[1]{z_{#1}}

\newcommand{\setpwins}[3]{#3^{#2}_{#1}}

\newenvironment*{caselist}[1][- Case]{%
    \newcommand{\case}[1]{\item[\noindent\emph{#1 ##1}:]}
    \begin{inparaitem}
        }{%
    \end{inparaitem}
}

\newenvironment*{axcaselist}[1][- Case]{%
    \newcommand{\case}[1]{\item[\noindent{#1 ##1}:]}
    \begin{inparaitem}
        }{%
    \end{inparaitem}
}

\newcommand{\sidecon}{\ensuremath{\dagger}}
\newcommand{\sideconb}{\ensuremath{\ddagger}}

\newcommand{\gsnotb}[1]{{#1}^{\tilde{\mathsf{d}}}}

\newcommand{\gatomvec}[1][\gatom]{\mathbf{#1}}
\newcommand{\gatomvece}[2][\gatom]{#1_1,\ldots,#1_{#2}}

% \newcommand{\sabset}[2][\gatom]{\chi_{\gatomvec[#1]}(#2)}
\newcommand{\sabsetnv}[2][\gatom]{#1{:=}#2}
\newcommand{\sabset}[2][\gatom]{\gatomvec[#1]{:=}#2}
\newcommand{\sabreadnv}[2][\gatom]{?#1{=}{#2}}
\newcommand{\sabread}[2][\gatom]{?\gatomvec[#1]{=}{#2}}

\newcommand{\sabsettruenv}[1]{#1!}
\newcommand{\sabsetfalsenv}[1]{\fnot#1!}
\newcommand{\sabsettruefalsenv}[1]{\pm#1!}
\newcommand{\sabreadtruenv}[1]{?#1}
\newcommand{\sabreadfalsenv}[1]{?\fnot#1}

\newcommand{\sabreadfalsedualnv}[1]{?^{\raisebox{2pt}{$\scriptscriptstyle\gduals$}}\kern-3pt#1}
\newcommand{\sabreadtrueedualnv}[1]{?^{\raisebox{2pt}{$\scriptscriptstyle\gduals$}}\kern-3pt{\fnot}#1}

\newcommand{\sabreadfalsedual}[1]{\sabreadfalsedualnv{\mathbf{#1}}}
\newcommand{\sabreadtrueedual}[1]{\sabreadtrueedualnv{\mathbf{#1}}}
% \newcommand{\sabreadtrueedualnv}[1]{?^{\scriptscriptstyle \gduals}\kern-3pt{\fnot}#1}
% \newcommand{\sabreadfalsedualnv}[1]{?^{{}^{\gduals}}\kern-4pt#1}

\newcommand{\sabsettrue}[1]{\sabsettruenv{\mathbf{#1}}}
\newcommand{\sabsetfalse}[1]{\sabsetfalsenv{\mathbf{#1}}}
\newcommand{\sabsettruefalse}[1]{\sabsettruefalsenv{\mathbf{#1}}}
\newcommand{\sabreadtrue}[1]{\sabreadtruenv{\mathbf{#1}}}
\newcommand{\sabreadfalse}[1]{\sabreadfalsenv{\mathbf{#1}}}

\newcommand{\svtrue}{\ftrue}
\newcommand{\svfalse}{\ffalse}

\renewcommand{\gmod}[1]{\mathsf{#1}}


\newcommand{\rlglmutail}[2][U]{{#2}_{#1}}
\newcommand{\rlglmutailp}[2][U]{({#2})_{#1}}
\newcommand{\rlglmutoexpglmodp}[1]{\rlglmutoexpglmod{(#1)}}

\newcommand{\tdgatomvec}{\gatomc}
\newcommand{\tdgatombvec}{\gmod{\gvar}}
\newcommand{\tdgatombvecz}{\gmod{\gvarz}}
\newcommand{\gvarlem}{\gvarc}

% \newcommand{\repdot}{\usebox{\USarg}}
% \newcommand{\repdot}{{\boldsymbol{\cdot}}}
\newcommand{\repdot}{{\text{\textbullet}}}

\newcommand{\contvarrep}{\contvar{\repdot}}
\newcommand{\contrep}{\cont_{\repdot}}
\newcommand{\gvarrep}{\gvar_{\repdot}}

\newcommand{\Andre}{Andr{\'{e}}}
\newcommand{\Beckic}{Becki{\'{c}}}

\newcommand{\dedisj}[1]{{#1}^{\for}}
\newcommand{\dedisjp}[1]{{(#1)}^{\for}}

\newcommand{\rdisjvar}{\pvar}

\newcommand{\contlist}{d}
\newcommand{\scvars}{g}
\newcommand{\scvar}{\gatomvec[\scvars]}
% \newcommand{\cont}{def}

\newcommand{\freplacea}[3]{C(#3)}

\newcommand{\gdornot}[1]{#1^{\pm\gduals}}
\newcommand{\gdualpot}[1]{(#1)^{\pm\gduals}}
\newcommand{\gesabotage}[1]{{\sim}{#1^{\pm\mathrm{d}}}}
\newcommand{\ganyterm}{{\gtest{\ffalse}}^{\color{gray}\mathrm{d}}}

\newcommand{\contextse}[3]{\contexts_{#1}^{#2=#3}}
\newcommand{\contextsesub}[3]{\contexts_{#1}^{#2=#3}}
\newcommand{\playervar}{p}

\newcommand{\sabsym}{{\sim}}
\newcommand{\dsabsym}{\kern1pt\rotatebox{90}{\kern-0.5pt$\sabsym$}}

\newcommand{\doubsabsym}{\approx}
\newcommand{\ddoubsabsym}{\kern1pt\rotatebox{90}{\kern-0.5pt$\doubsabsym$}}
% \newcommand{\dsabsym}{{\gdual{\sim}}}


\newcommand{\localcont}{C}

\newcommand{\localcontname}{formula-context\xspace}

\newcommand{\gamcont}{\Omega}

\newcommand{\correcttranslation}[1]{#1 Sound}
\newcommand{\correcttransformation}[1]{#1 Transformation}
\newcommand{\provablecorrectnessrgl}{Provable Inverses}
\newcommand{\provablecorrectnessgls}{Provable Inverse}
\newcommand{\semanticroundtrip}{Semantic Inverses}

\definecolor{vblue}{rgb}{.08,.15,.62}
\definecolor{vvblue}{rgb}{.14,.21,.868}%{1.4*vblue} % axkeycolor

% \colorlet{emphcolor}{ACMPurple}
% \colorlet{emphcolor}{ACMLightBlue}
% \colorlet{emphcolor}{ACMBlue} 
\colorlet{emphcolor}{ACMDarkBlue}
% \colorlet{emphcolor}{vblue}

% \newcommand{\cev}[1]{\overleftarrow{#1}}
\newcommand{\cev}[1]{\reflectbox{$\,\vec{\reflectbox{$#1$}}\,$}}

\newcommand{\ggsnot}[1]{\gsnot{\gsnot{#1}}}
\newcommand{\ffsnot}[1]{{\fsnot{\fsnot{#1}}}}

\newcommand{\contextsb}{\mathcal{D}}

\newcommand{\rankless}{\prec}
